SeMoLi: What Moves Together Belongs Together

We tackle semi-supervised object detection based on motion cues. Recent results suggest that heuristic-based clustering methods in conjunction with object trackers can be used to pseudo-label instances of moving objects and use these as supervisory signals to train 3D object detectors in Lidar data without manual supervision. We re-think this approach and suggest that both, object detection, as well as motion-inspired pseudo-labeling, can be tackled in a data-driven manner. We leverage recent advances in scene flow estimation to obtain point trajectories from which we extract long-term, class-agnostic motion patterns. Revisiting correlation clustering in the context of message passing networks, we learn to group those motion patterns to cluster points to object instances. By estimating the full extent of the objects, we obtain per-scan 3D bounding boxes that we use to supervise a Lidar object detection network. Our method not only outperforms prior heuristic-based approaches (57.5 AP, +14 improvement over prior work), more importantly, we show we can pseudo-label and train object detectors across datasets.

==> sec/6_acknowledgement.tex <==
\vspace{+0.2cm}
\noindent\textbf{Acknowledgments:} We thank OC Kush for his mental support and the KVR for useful discussions.

==> tables/PC_FILTERING_ORACLE.tex <==
\begin{table}[htp!]
    \centering
    \caption{\textbf{Oracle pseudo-label quality of ground truth bounding boxes with respect to the number of interior points $ \geq x_f$ after point cloud filtering:}} 
    \footnotesize
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
    \toprule
        Method & Pr & Re & AP \\
        \hline\hline
        $x_f=0$ & 1.0 & 1.0 & 1.0 \\ 
        $x_f=10$ & 1.0 & 81.0 & 81.0 \\ 
        $x_f=30$ & 1.0 & 71.0 &  71.0 \\ 
        $x_f=50$ & 1.0 & 61.0 &  61.0 \\ 
    \bottomrule
    \end{tabular}
   %}
    \label{tab:oracle_num_interior}
\end{table}


==> tables/PLQ_CLASS_WISE_ARGO_LONG.tex <==
\begin{table}[htp!]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{5pt}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|cccc}
    \toprule
         & \multicolumn{2}{c}{\textit{3DIoU}}  & \multicolumn{2}{c}{\textit{SegIoU}} \\
         & Re (Pr) 0.7 & Re (Pr) 0.4 & Re (Pr) 0.7 & Re (Pr) 0.4 \\
        \midrule
        \textit{Ours} \\
        Bicycle + Bicyclist & -  & 56.3 & -&   86.4 \\
        Box Truck & -&  0 & -&  44.5 \\
        Bus & -&   0.4 & -&  39.3 \\
        Large Vehicle & - & 17.1 &-&   44.4 \\
        Motorcyclist & -&   100 & -&  100 \\
        Pedestrian & -&   42.5 & -&  57.1\\
        Regular Vehicle &-& 56.9 &-&   77.9 \\
        Stroller & -&   0.5  &-&   0.5 \\
        Truck & -&   4.4 &-&   94.1 \\
        Vehicular Trailer & -&   0& -&   14.0 \\
        \midrule
        Class-agnostic &  & 45.8 (40.1) &  & 65.2(57.0) \\
        \midrule
        \midrule
        \textit{DBSCAN++$^{\dagger}$} \\
        Bicycle + Bicyclist & - & 35.9 & - & 70.9 \\
        Box Truck & - & 5.8 & -&  61.3 \\
        Bus & - & 0.4 &-&   28.0 \\
        Large Vehicle & - & 6.4 &-&   33.8 \\
        Motorcyclist & - & 52.6 & -&   52.6 \\
        Pedestrian & - & 25.5 & -&  48.9 \\
        Regular Vehicle & - & 46.2 & -&  73.6 \\
        Stroller & - & 0 & - & 0 \\
        Truck & - & 0 &-&   95.6 \\
        Vehicular Trailer & - & 5.3 &-&   19.3 \\
        \midrule
        Class-agnostic &   & 32.9 (11.4) &  & 56.0 (19.3) \\
    \bottomrule
    \end{tabular}
   }
    \caption{\textbf{Generalization of our GNN to new classes and sensors:} We evaluate our approach trained on 90\% labeled Waymo Open Dataset on Argoverse2 dataset. Note that we never train our approach on Argoverse2. We obtain the flow in the same unsupervised way as for Waymo open dataset. We also report results for DBSCAN++$^{\dagger}$.} 
    \label{tab:av2_performance}
\end{table}

==> tables/PLQ_CLASS_WISE_WAYMO_LONG.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{5pt}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|cc|cc|c}
    \toprule
        & \multicolumn{2}{c}{\textit{3DIoU}}  & \multicolumn{2}{c}{\textit{SegIoU}} & \\
         & Re 0.3 & Re 0.4 & Re 0.3 & Re 0.4 & uFP \\
        \midrule
        DBSCAN++$^{\dagger}$ Vehicle &  & 39.7 & & &  \\
        DBSCAN++$^{\dagger}$ Pedestrian &  & 46.5 & & &  82.5 \\
        DBSCAN++$^{\dagger}$ Cyclist &  & 79.2 & & &  \\
        \hline
        % 10% labeled
        % Ours Vehicle & 31.9 & 54.9 & 66.5 & 2343 \\
        % Ours Pedestrian & 14.6 & 42.8 & 55.9 & 2343 \\
        % Ours Cyclist & 60.4 & 79.2 & 91.7 & 2343 \\
        % 90% labeled
        Ours Vehicle & & 64.3 & & & \\
        Ours Pedestrian &  & 54.7 & &  & 23.8 \\
        Ours Cyclist &  & 75.0 & & & \\
    \bottomrule
    \end{tabular}
   }
    \caption{\textbf{Class-wise evaluation of pseudo-labels:} We match pseudo-labels to ground truth bounding boxes based on a 3D bounding box IoU of 0.99. We then assign each pseudo-label the class of the corresponding bounding box. If a pseudo-label can not be matched we consider it as unmatched false positive which we report relative to all pseudo-labels in $\%$ (uFP).} 
    \label{tab:class_wise}
\end{table}

